Infused Suppression Of Magnification Artefacts For Micro-AU Detection

Facial micro-expressions are spontaneous, brief and subtle facial motions that unveil the underlying, suppressed emotions. Detecting Action Units (AUs) in micro-expressions is crucial because it yields a finer representation of facial motions than categorical emotions, effectively resolving the ambiguity among different expressions. One of the difficulties in micro-expression analysis is that facial motions are subtle and brief, thereby increasing the difficulty in correlating facial motion features to AU occurrence. To bridge the subtlety issue, flow-related features and motion magnification are a few common approaches as they can yield descriptive motion changes and increased motion amplitude respectively. While motion magnification can amplify the motion changes, it also accounts for illumination changes and projection errors during the amplification process, thereby creating motion artefacts that confuse the model to learn inauthentic magnified motion features. The problem is further aggravated in the context of a more complicated task where more AU classes are analyzed in cross-database settings. To address this issue, we propose InfuseNet, a layer-wise unitary feature infusion framework that leverages motion context to constrain the Action Unit (AU) learning within an informative facial movement region, thereby alleviating the influence of magnification artefacts. On top of that, we propose leveraging magnified latent features instead of reconstructing magnified samples to limit the distortion and artefacts caused by the projection inaccuracy in the motion reconstruction process. Via alleviating the magnification artefacts, InfuseNet has surpassed the state-of-the-art results in the CD6ME protocol. Further quantitative studies have also demonstrated the efficacy of motion artefacts alleviation.

==> tex/archiveText.tex <==
% % talk about what we are proposing here as solutions to the problem
% % we are proposing mixup
% To solve the class imbalance problem, we propose adapting the manifold mixup algorithm to augment the smaller AU classes \cite{zhang2017mixup}. 

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{images/methodology/mmew_samples.PNG}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}

% % we are proposing merging magnification into optical flow
% Next, we adapted the learnable magnification \cite{oh2018learning} along with optical flow \cite{sun2010secrets} for feature extraction. As micro-expression appears subtle, using RGB frames for feature extraction is less ideal and optical flow is sought after because it extracts the shape representation and motion changes of micro-expression. Despite that, optical flow may still have limitations in extracting extremely tiny facial motions. In another aspect, motion magnification has the capability in increasing the amplitude of motion changes with a cost of motion artefacts. Therefore, there exists a symbiotic relationship between optical flow and motion magnification, where optical flow filters off additional motion artifacts and leads to a better feature extraction process. 


% % talk about Mixup and weightage
% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\linewidth]{images/methodology/manifoldMixup.PNG}
%     \caption{The illustration of our adaptation of mixup algorithm to regularize the feature learning process to inculcate class imbalance learning problem. }
%     \label{fig:manifold_mixup}
% \end{figure}

% The proposed framework is two-fold: (1) model fusion to cross-compensate between magnified and motion information.
% (2) manifold mixup to increase the intermediate representation of samples, thus bridging the gap between small and big AU Classes.

% \subsection{Manifold Mixup}
% As some AUs naturally tend to be rarer in occurrence, the data distribution across different AU classes is imbalanced as demonstrated in Table \ref{tab:au_distribution}. Hence, it complicates the feature learning process and creates a feature bias for bigger AU classes. Thus, we propose adapting the Mixup algorithm to augment samples residing in small AU Classes to balance the feature learning process. We define AU Classes with sample percentages less or equal to 10\% as smaller AU classes. 

% Figure \ref{fig:manifold_mixup} illustrates that we first select samples with labels in smaller AU classes. Then, we pair them in two ways:
% \begin{itemize}
%     \item Pairing smaller classes with each other. ($X_{i, small}$ - $X_{j, small}$, $y_{i, small}$ - $y_{j, small}$)
%     \item Pairing smaller classes with one randomized big class. ($X_{i, small}$ - $X_{j, big}$, $y_{i, small}$ - $y_{j, big}$)    
% \end{itemize}

% In every iteration, we sample from Dirichlet Distribution with a random number, $\lambda$ which will determine the intermediate values between $(X_{i}, y_{i})$ and $(X_{j}, y_{j})$ and the intermediate values will be the augmented samples. The equations for $x$ and $y$ are demonstrated in Equation \ref{eq:mixup_x} and \ref{eq:mixup_y} respectively. 

% \begin{equation}
%     \Tilde{x} = \lambda x_{i} + (1 - \lambda) x_{j}
%     \label{eq:mixup_x}
% \end{equation}
% \begin{equation}
%     \Tilde{y} = \lambda y_{i} + (1 - \lambda) y_{j}
%     \label{eq:mixup_y}
% \end{equation}

% \begin{table*}[ht]
%     \centering
%     \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
%         \hline
%          AU1 & AU2 & AU4 & AU5 & AU6 & AU7 & AU9 & AU10 & AU12 & AU14 & AU15 & AU17 & Total \\
%          \hline
%         304 & 280 & 708 & 134 & 60 & 252 & 117 & 75 & 176 & 277 & 52 & 86 & 2521    \\         
%         (12\%) & (11\%) & (28\%) & (5\%) & (2\%) & (10\%) & (5\%) & (3\%) & (7\%) & (11\%) & (2\%) & (3\%) & 100\% \\
        

%         \hline
%     \end{tabular}
%     \caption{Data distribution of AU Classes}
%     \label{tab:au_distribution}
% \end{table*}


==> tex/introduction.tex <==
% % \vspace{-2em}
\section{Introduction}
\label{sec:intro}
% BAckground
Micro-expressions are spontaneous, subtle and rapid (1/25 to 1/3 seconds) facial movements solicited under high-stakes environments \cite{ekman1971constants} \cite{ekman2009lie} such as psychological diagnosis, interviews and interrogations. In micro-expression analysis, detecting Action Units (AUs) is critical as it yields a finer granularity in micro-facial motion analysis than recognizing emotions and reduces the ambiguity in analyzing individual emotion \cite{niu2019local}. Thus, it is garnering attention in affective computing research despite its challenges.

% Problem
One of the critical challenges of micro-expression analysis is the subtle motion. Consequently, motion magnification \cite{oh2018learning} has been utilized to amplify the magnitude of the motion changes. In micro-expression AU detection, several works \cite{li2021intra} \cite{li2021micro} \cite{wei2023cmnet} have proposed incorporating motion-magnified video frames for AU detection. However, while facial muscle movements are amplified to enhance visibility, it inadvertently amplifies noise (e.g., from external factors such as illumination), creating facial distortions. Meanwhile, the reconstruction of magnified motion also contributes to the facial distortions due to the inaccurate projection, as illustrated in Figure \ref{fig:concept} (A). The motion artefacts can be detrimental in fine-grained AU detection task, which motivates us to study the alleviation of artefacts.

% Despite that, the motion artefacts are understudied as its influence to the performance is minimal. It can be increasingly critical as the task gets complicated, such as AU detection in cross-database problems. This prompts us to study the removal of magnification artefacts in this work. 

% % Solution
% Given the presence of scattered magnification artefacts, obtaining a cleaner magnified signal requires a guided approach that prioritizes regions with motion while suppressing those without. For that, optical flow and optical strain have been widely utilized in this domain \cite{liu2015main} \cite{gan2019off} \cite{liong2015subtle} due to the precision in identifying facial motions. 

To address the aforementioned problems, we propose a framework known as \textbf{InfuseNet}, a unitary successive feature infusion technique that utilizes precise motion features to alleviate motion artefacts, as demonstrated in Figure \ref{fig:concept}. The motion features help to prioritize regions with motion in the presence of scattered magnification artefacts. For that, optical flow and optical strain are utilized due to the precision in identifying facial motions \cite{liu2015main} \cite{gan2019off} \cite{liong2015subtle}. Besides, we propose extracting the latent magnified features to minimize the motion artefacts generated from motion decoding. The extracted latent magnified features are then used directly as the input to a learnable feature encoder to learn the magnified motions. 




\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/conceptB.pdf}
    % \vspace{-5em}  
    \caption{The illustrations of magnification artefacts and feature infusion. Part (A) demonstrates the magnification artefacts generated during the motion amplification process, where faces appear deformed. Part (B) presents the proposed feature infusion process, which extracts latent magnified features while counterbalancing the amplified noise using optical flow images.}
    % \vspace{-5em}
    \label{fig:concept}
\end{figure}
% \vspace{-8em}



\begin{figure*}[!h]
    \centering
    \includegraphics[width=1.0\linewidth]{images/framework.pdf}
    % \vspace{-1.5em}

    \caption{Our proposed framework, InfuseNet alleviates the magnification artefacts via infusing motion context from FrameFlow. Given onset, apex and pseudo-apex frames, we extract the magnified latent features as the input to the FrameMag network. Whereas for FrameFlow, we extract the optical flow and strain features from the onset to apex frames. Following that, we perform successive layer feature infusion from FrameFlow to FrameMag, and then FrameMag predicts the eventual one-hot AUs of the samples.}
    % \vspace{-2.0em}
    \label{fig:framework}
\end{figure*}




In summary, our contributions are as follows:
\begin{itemize}
    \item Leveraging unitary successive layer features to alleviate magnified motion artefacts.
    \item Utilizing latent magnified features to minimize the motion artefacts generated from image decoding.
    \item Studying the problem of magnification artefacts and the effects artefacts removal on micro-AU detection with CD6ME protocol.    
\end{itemize}



% % \vspace{-1em}










